Few-shot Neural Radiance Fields Under Unconstrained Illumination

In this paper, we introduce a new challenge for synthesizing novel view images in practical environments with limited input multi-view images and varying lighting conditions. Neural radiance fields (NeRF), one of the pioneering works for this task, demand an extensive set of multi-view images taken under constrained illumination, which is often unattainable in real-world settings. While some previous works have managed to synthesize novel views given images with different illumination, their performance still relies on a substantial number of input multi-view images. To address this problem, we suggest ExtremeNeRF, which utilizes multi-view albedo consistency, supported by geometric alignment. Specifically, we extract intrinsic image components that should be illumination-invariant across different views, enabling direct appearance comparison between the input and novel view under unconstrained illumination. We offer thorough experimental results for task evaluation, employing the newly created NeRF Extreme benchmark-the first in-the-wild benchmark for novel view synthesis under multiple viewing directions and varying illuminations.

==> table/supple/extreme_6v.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{Cafe} & \multicolumn{3}{c|}{Kitchen} & \multicolumn{3}{c}{Flower}\\ \midrule
  & SSIM $\uparrow$ & LPIPS $\downarrow$ & Abs Rel $\downarrow$ & SSIM $\uparrow$& LPIPS $\downarrow$ & Abs Rel $\downarrow$ & SSIM $\uparrow$& LPIPS $\downarrow$ & Abs Rel $\downarrow$\\ \midrule
NeRF-W~\cite{nerfinthewild} \ & - & - & -  & - & - & - & - & - & - \\
Ha-NeRF~\cite{HaNeRF} \ & - & - & -  & - & - & - & - & - & - \\
\midrule
RegNeRF~\cite{niemeyer2022regnerf}\ & 0.45 & 0.41 & 0.91  & 0.55 & 0.40 & 0.85 & 0.53 & 0.49 & 0.91 \\
FreeNeRF~\cite{yang2023freenerf} \ & 0.45 & 0.42 & 0.91  & 0.54 & 0.40 & 0.81 & 0.51 & 0.47 & 0.86 \\
\midrule
NeROIC-Geom.~\cite{kuang2022neroic}\ & - & - & -  & - & - & - & - & - & - \\
%\midrule
\textbf{ExtremeNeRF (Ours)}\ & 0.49 & 0.37 & 0.91 & 0.61 & 0.35 & 0.79 & 0.58 & 0.42 & 0.84 \\
\bottomrule
\end{tabular}
